Precision measurements of jet and photon production at ATLAS

The production of jets and prompt isolated photons at hadron colliders provides stringent tests of perturbative QCD. The latest measurements performed by the ATLAS Collaboration at the LHC are presented in these proceedings. The inclusive prompt-photon production is measured for two distinct photon isolation cones, $R = 0.2$ and $0.4$, as well as for their ratio. This measurement is sensitive to the gluon parton density distribution in the proton. In addition, a measurement of variables probing the properties of the multijet energy flow which are used to determine the strong coupling constant is presented. These measurements are compared to state-of-the-art NLO and NNLO predictions. Lastly, a measurement of new event-shape jet observables defined in terms of reference geometries with cylindrical and circular symmetries using the energy mover's distance is discussed.

==> Sections/Summary.tex <==
Measurements of the inclusive isolated-photon production cross section and of event shapes probing the properties of the multijet energy flow in $pp$ collisions at $\cme = 13$~TeV recorded by the ATLAS experiment at the LHC are presented based on $\thirdlumi$ of $2015-2018$ data.

The dependence on $R$ of the inclusive isolated-photon cross sections is measured for first time, and found to be well described by the NLO \jetphox and NNLO \nnlojet pQCD predictions. The ratios of differential cross sections provide a very stringent test of pQCD, with significantly reduced experimental and theoretical uncertainties, and validate the underlying theoretical description up to $\mcal{O}(\alphas^2)$.

The measurement of transverse energy–energy correlations and their corresponding asymmetries bennefit from the inclusion of NNLO QCD corrections to three-jet production in the theoretical predictions for the first time, allowing a reduction by a factor of 3 of the theoretical uncertainties in both the cross-section calculation for the TEEC and ATEEC distributions and in the determination of the strong coupling constant $\alphas$.

A first application of optimal transport techniques in a collider physics measurement is performed in the measurement of the multijet event isotropies. The measured data are compared with the predictions of several state-of-the-art Monte Carlo event generators. Agreement between the unfolded data and the simulated events tends to be best in balanced, dijet-like arrangements and deteriorates in more isotropic configurations.
